Causality for Natural Language Processing

Causal reasoning is a cornerstone of human intelligence and a critical capability for artificial systems aiming to achieve advanced understanding and decision-making. This thesis delves into various dimensions of causal reasoning and understanding in large language models (LLMs). It encompasses a series of studies that explore the causal inference skills of LLMs, the mechanisms behind their performance, and the implications of causal and anticausal learning for natural language processing (NLP) tasks. Additionally, it investigates the application of causal reasoning in text-based computational social science, specifically focusing on political decision-making and the evaluation of scientific impact through citations. Through novel datasets, benchmark tasks, and methodological frameworks, this work identifies key challenges and opportunities to improve the causal capabilities of LLMs, providing a comprehensive foundation for future research in this evolving field.

==> Minimals/Info.tex <==
\thispagestyle{empty}

\begin{center}
\vspace*{2cm}
\noindent
\centering{\titlefont{Causal Inference for \\ Natural Language Processing}}

\vspace*{3cm}
\begin{minipage}{\linewidth}

\centering \printauthor
\vspace*{1.8cm}

%\includegraphics[scale=1]{Logos/logo_un.jpg}\\
\fontsize{13pt}{13pt} \selectfont 
June 2024

\vspace{1.8cm}
Department of Computer Science\\
\vspace{0.1cm}
Faculty of Science\\
\vspace{0.1cm}
University of Tuebingen, Germany\\
\vspace{2.5cm}

\textsc{Thesis Committee:}\\
\vspace{0.1cm}
 Prof. Dr. Bernhard Schölkopf \\
 Prof. Dr. Matthias Bethege \\
 Prof. Dr. Mrinmaya Sachan \\
 Prof. Dr. Rada Mihalcea \\
% \scshape
% Universidad Nacional de Colombia
\vspace{3cm}



\fontsize{12pt}{12pt}\selectfont \text{Submitted in partial fulfillment of the requirements for the degree of}\\
\vspace{0.1cm}
\fontsize{12pt}{12pt}\selectfont \textbf{Doctor of Philosophy in Computer Science}\\
\end{minipage}

\vfill
© 2024, Zhijing Jin. All rights reserved.
\end{center}

==> Minimals/Title_original.tex <==

\clearpage





\begin{titlepage}
\vspace*{2cm}
\noindent
\centering{
% \baselineskip=1.5\baselineskip
\titlefont{Causal Inference for \\
Natural Language Processing}
}


\vspace*{5cm}
\begin{minipage}{\linewidth}

\centering  \printauthor
\vspace*{5cm}

% \includegraphics[scale=1]{Logos/logo_un.jpg}\\
\fontsize{13pt}{13pt}\selectfont Faculty of Science\\
\vspace{0.1cm}
Department of Computer Science\\
\vspace{0.1cm}
University of Tuebingen, Germany\\
\vspace{0.1cm}
June 1, 2024
\end{minipage}
\end{titlepage}

